Challenging the Semi-Supervised VAE Framework for Text Classification

Semi-Supervised Variational Autoencoders (SSVAEs) are widely used models for data efficient learning. In this paper, we question the adequacy of the standard design of sequence SSVAEs for the task of text classification as we exhibit two sources of overcomplexity for which we provide simplifications. These simplifications to SSVAEs preserve their theoretical soundness while providing a number of practical advantages in the semi-supervised setup where the result of training is a text classifier. These simplifications are the removal of (i) the Kullback-Liebler divergence from its objective and (ii) the fully unobserved latent variable from its probabilistic model. These changes relieve users from choosing a prior for their latent variables, make the model smaller and faster, and allow for a better flow of information into the latent variables. We compare the simplified versions to standard SSVAEs on 4 text classification tasks. On top of the above-mentioned simplification, experiments show a speed-up of 26%, while keeping equivalent classification scores. The code to reproduce our experiments is public.

==> djame_linguistics.tex <==
\paragraph{Linguistics information in neural models} \draftHL{Such parallels}{what paralells? -ds} provide better inductive bias in NLP machine learning systems.
 RNNG \cite{Dyer2016RecurrentGrammars}, ON-LSTM \cite{Shen2019OrderedNetworks}, ONLSTM-SYD \cite{Du2020ExploitingApproach},
  and SIVAE \cite{Zhang2020Syntax-infusedGeneration} are examples among others of successful attempts at \draftreplace{having linguistic 
  information appear}{showing how linguistic information is captured} in a neural language model. 
  Many ensuing works 
have also dived into their linguistic capabilities, the types of linguistic annotations that emerge best in them, and syntactic error
analysesn(\citealp{Hu2020AModels}, \citealp{Kodner2020OverestimationModels}, \citealp{Marvin2020TargetedModels},
   \citealp{Kulmizev2020DoFormalisms}). BERT \cite{Devlin2018} has, in turn, been subject to studies showing \draftreplace{it operates on
sentences as would}{that the linguistics information it captures are organized among its layers in a way remarkably close to the way} a classical NLP pipeline \draftadd{works} \cite{Tenney2020BERTPipeline}. \draftadd{Furthermore, many other authors, among which \cite{Clark2019WhatAttentionb}, showed that it was possible to extract accurate dependency based-representations from its attention heads. We refer to the reader to  \cite{Rogers2020AWorks} for an extensive review of Bert-related studies.} However, most of those studies mostly rely on \draftadd{structural} probes to explain representations, probes which are not without issues as shown by  \citet{Pimentel2020Information-TheoreticStructure} 
who exposed some of this methodology's "fundamental flaws", and which is, according to them, often misused. \draftadd{In that aspect,} we believe the generative capabilities and the attention mechanism \draftreplace{in}{of} our model offer a \draftadd{natural}{interesting and intuitive} alternative to probing.

\draftremove{and that its attention heads perform impressively
well at dependency parsing \cite{Clark2019WhatAttentionb}. \citealp{Rogers2020AWorks} offer an  review of BERT-related studies.}


==> draft_final.tex <==
\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
  \do\Y\do\Z}


%\captionsetup{belowskip=0pt}

\usepackage{soulutf8}
\usepackage[normalem]{ulem}
\usepackage{xcolor}

% to reduce space between items (djame)
\usepackage{enumitem}
\setlist{nolistsep}
\usepackage{microtype}

\iffalse % set to iftrue for camera ready version, iffalse to display draft comments
    \usepackage[final]{proofing}
  \renewcommand\hl[1]{{#1}}  %% to remove the highlith
   \newcommand\draftHL[2]{#1}{\draftnote{\red{#2}}}
   \newcommand\redHL[1]{}
  \newcommand\todo[1]{}
  %\aclfinalcopy % Uncomment this line for the final submission
  
  
  \newcommand{\Djame}[1]{}
  \newcommand{\GW}{}
\newcommand{\Jose}{}


%\pagestyle{plain} % just so we can see the pagenumber

\else  % the stuff below is for the draft mode (hl, comments and so)
%% this in order to see the margin note
 %% will go back to normal for the submitted version

%\usepackage[a4paper,left=2cm,right=2m]{geometry}
\setlength{\marginparwidth}{1.2cm}

\usepackage[draft]{proofing}

\newcommand\hlr[1]{\textbf{\textcolor{red}{\hl{ #1}}}}

\newcommand{\Djame}[1]{
\textbf{\textcolor{red}{\hl{Djame: #1}}}
}

\newcommand{\GW}[1]{
\textbf{\textcolor{red}{\hl{GW: #1}}}
}


\newcommand{\Jose}[1]{
\textbf{\textcolor{red}{\hl{GW: #1}}}
}


\newcommand\red[1]{{{\textcolor{red}{\bf #1}}}}
\newcommand{\barre}[1]{
 {\textcolor{red}{{\sout{#1}}}}}

\newcommand\draftHL[2]{\hl{#1}{\draftnote{\red{#2}}}}


\let\oldred\red
\renewcommand\red[1]{{ \oldred{{#1}}}}
\renewcommand{\barre}[1]{
 {\textcolor{red}{{\sout{#1}}}}}

 \renewcommand\draftHL[2]{\hl{#1}{\draftnote{\red{#2}}}}
 \newcommand\redHL[1]{\red{\hl{#1}}}
%  \renewcommand\todo[1]{\draftnote{#1}}
\let\olddraftnote\draftnote
\renewcommand\draftnote[1]{\olddraftnote{\red{#1}}}
\newcommand\remarq[1]{\draftnote{#1}}

%\pagestyle{plain} % just so we can see the pagenumber
\fi



\newcommand\ie{{\textit{ i.e }\xspace}}
\newcommand\eg{{\textit{ e.g }\xspace}}

